Fractal dimension of a liquid flows predicted coupling an Eulerian-Lagrangian approach with a Level-Set method

The fractal dimension of a liquid column is a crucial parameter in several models describing the main features of the primary break-up occurring at the interface of a liquid phase surrounded by the gas-flow. In this work, the deformation of the liquid phase has been numerically studied. The gas-phase is computed as a continuum in an Eulerian frame while the liquid phase is discretized in droplets Lagrangian tracked and coupled via the momentum equation with the surrounding gas flow. The interface is transported by the flow field generated because of the particle forcing and it is numerically computed using the Level-Set method. Finally, the fractal dimension of the interface is locally estimated and used as criterion for the model of the primary breakup.

==> Introduction.tex <==
\section{Introduction}


The atomization of a liquid jet is a crucial process in combustion, exhaust gas post-treatment systems 
and other devices. 
The phenomenon of the primary breakup for the application to selective catalytic reduction (SCR) has been analysed according to
the following set-up:



\begin{figure}[!h]
\begin{center}
\includegraphics[width=.2\textwidth,angle=0]{./figs/poster1.png}
\caption{\small Schematic of the injector and of the spray.}
\label{fig:poster1.png}
\end{center}
\end{figure}




\begin{table}[!h]
\begin{center}
\begin{tabular}{ll}
\hline
Simulation of ADBLUE (urea/water) sprays for SCR use\\
\hline
\hline
Number of holes:& 3\\

Holes diameter: &0.123 [mm]\\

Lenght/diameter & 0.5\\

Injection pressure: &7.5 [bar]\\

Mass flow per hole:& 3.33e-04 [kg/s]\\

Cone angle: & $4^o$\\

fluid:& water\\
\hline
\end{tabular}
\end{center}
\caption{\small Set-Up for the ADBLUE spray.}
\end{table}




The evaporation velocity of a liquid jet increase if the jet is atomizated because of the greater ratio between the surface
and the volume of the liquid phase.

The liquid jet fragments up to evaporate according with two main mechanisms: the primary and the secondary breakup.
Firstly, coherent structures detach from the jet up to break in spherical droplets because 
of either the Rayleigh-Taylor or Kelvin-Helmholtz instability on the liquid/gas interface
 (primary breakup). 
 The interface instability is locally modulated by waves with a critical wave-length and magnitude.
This phenomenon enhance for increasing the turbulence since the velocity and the pressure fluctuations are extended to
the smaller length scales.
Thus, each droplet, occurring in the primary breakup, fragments up to evaporate because of the shear stress induced by the surrounding flow 
(secondary breakup).

Understanding and prediction of spray breakup plays
a leading role in the design of injector.
In this scenario, numerical simulations are suitable to analyze this process more in detail than  the ensemble description   
 provided by experiments.
The numerical description of the jets dynamics involve both the solution of the governing equation of each phase and the 
 topological  treatment of the fluid-gas interface. 

In the past years, the research focused on the numerical methods for the interface tracking of incompressible multi-phase flows.
The Front Tracking \cite{Front1}, the Volume of Fluid method 
\cite{Vol1} and the Level-Set \cite{Level1} are  the most remarkable techniques used in literature.

The Front Tracking method is based on the Lagrangian treatment of the interface that is described by ideal particle (markers). 
The markers are connected each other and they are moved like an ideal fluid particle. The connectivity between discrete elements 
covering the interface is not straightforward in three spatial dimensions.
The drawback of this method depends on the collapsing, the stretching and the deformation of some discrete elements. These elements should be periodically
replaced in order to preserve the  curvature and the mass of the fluid confined by the interface.
These difficulties vanish if the interface is described using methods in the Eulerian frame as the Volume of Fluid method or the Level-Set method. 

In the Volume of Fluid method each phase is represented by the volume
fraction of the fluid per each computational cell and the interface evolves according to the advection equation. 
Despite of the simplicity in describing the connectivity,   
 a thickness of the interface is artificially introduced.     
Thus, the curvature and the surface tension are not well estimated. The advantage of this method consists in the accurate mass conservation.

With the Level-Set method the interface is described  by the iso-contour of an implicit function whose evolution is governed by the 
advection equation in a fixed computational grid. The implicit function ensure the description of complex gas-fluid interface 
without the stringent conditions coming from the parametric representation of the surface.
With the Level-Set method the interface is well defined and the surface tension is precisely predicted.
Specifically, the most advantages of the implicit function are highlighted using the distance function defined as 
$\phi(\textbf{x})=min(\textbf{x}-\textbf{x}_i)$ where $\textbf{x}$ and $\textbf{x}_i$ are the points of the computational domain $\Omega$ 
and at the interface $\partial \Omega$Ω, respectively.
The interface, the outer region and the inner region are defined by 
$\phi(\textbf{x})=0$, $\phi(\textbf{x})>0$, $\phi(\textbf{x})<0$, respectively.
Under these assumption the normal to the interface is $\textbf{n}=\nabla\phi$  and the mean curvature is $k=(\nabla^2\phi)/2$.
The evolution of the interface is governed by the following equation:
	 $\phi_t+\textbf{u}\nabla\phi=0$, where $\textbf{u}$ is the flow velocity. 
Moreover, with the signed distance function it is easy to make the intersection and the union of two different region.
If $\phi_1$ e $\phi_2$ are two different distance function the union of the inner region is $\phi =min(\phi_1, \phi_2)$, while the intersection of 
the inner region is
 $\phi =max(\phi_1, \phi_2)$.

Once the interface location is known the  Navier-Stokes equation are solved into all the phases.
The jump condition is enforced as boundary condition into the computational cells containing the interface (ghost cells).
In the methods described above, the steep gradients of density and viscosity
 across the interface make tricky the fast simulation of such flows for high Reynolds numbers.
Indeed, the numerical simulation of the interface requires a massive computational cost  
to solve the governing equation in a refined grid.
This implies a restricted application range out of the industrial needs.
For this reason, most of the research focused on the models for the secondary atomization while the initial breakup is not well investigated.
For instance, the Enhanced Taylor Analogy Breakup (ETAB) model simulates the liquid jet disintegration process as a cascade of drop breakups.
The breakup criterion is determined by Taylor's linear drop deformation dynamics and the associated drop breakup condition.
Breakup occurs when the normalized drop distortion exceeds a critical value.
The breakup into product droplets is modelled after the experimentally observed bag or
stripping breakup mechanisms and the radial velocities of the product droplets are derived from an energy conservation consideration.

The aim of this research is to join the Level-Set method with the Two-way Lagrangian Particle Tracking for the simulation of
jets in turbulent flows.
The Level-Set is used like criterion to define the jet topology and to estimate the regions in which the primary breakup occurs according 
with the following steps:
\begin{enumerate}
\item Each particle is Lagrangian Tracked and it is coupled via momentum and energy equations with the surrounding fluid.
\item The interface is transported by the flow field generated by the particle forcing. 
\item The fractal dimension of the interface is locally estimated and used as criterion for the model of the primary breakup.
\end{enumerate}

In this way, the main features of the fluid dynamics are adequately captured in a fast fashion and the interface topology is 
precisely predicted for the whole simulation time. This tool is oriented to the industial needs of 
the fast and accurate prediction of the jet atomization.

Future developments of the project consist to apply the Refined Level Set Grid (RLSG) to the primary atomization problem.
This method, in a detached code, resolves and tracks all relevant phase interface length scales on a separate,
locally refined grid. The RLSG code is coupled to the flow solver via a multi-code coupling environment.











==> Lagrangian.tex <==
\subsection{Lagrangian particle tracking}
\label{LPT}
%%%%%%%%%%%

Lagrangian particle tracking is a methodology to describe the particle motion
computing  velocity and position for each particle \cite{Sq90,Elg93,Boi98}.
The particle equation is modulated by the following
control parameters that describe the main properties of the physical system:
response time, Stokes number, dilute versus dense flow.
The one-dimensional equation for a spherical particle with only steady drag force is
useful to describe the main features of the particle dynamics:

\begin{equation}\label{eq:partlib}
m_p\frac{dv}{dt}=\frac{1}{2}C_D\frac{\pi
d_p^2}{4}\rho_f|u-v|(u-v)
\end{equation}


We have indicate with: $m_p$ the mass,
$d_p$ the diameter,
$v$ the velocity of the droplet,  $u$ the flow velocity,
$t$ the time, $C_D$ the drag coefficient.

We can define the relative Reynolds number as:

\begin{equation}
Re_p=\frac{\rho_f d_p|u-v|}{\mu}
\end{equation}

where $\mu$ is the dynamic viscosity of the fluid. We can rearrange the equation (Eq. \ref{eq:partlib}) as follows:


\begin{equation}\label{eq:partlib2}
\frac{dv}{dt}=\frac{18\mu}{\rho_p
d_p^2}\frac{C_DRe_p}{24}(u-v)
\end{equation}


For the limits of low Reynolds number (Stokes flow), the factor $C_DRe_p/24$
approaches unity. In this case the equation (Eq. \ref{eq:partlib2})is governed
only by the response time
$\tau_p$:

\begin{equation}\label{eq:partlib3}
\frac{dv}{dt}=\frac{1}{\tau_p}(u-v);\hspace{1cm}\tau_p=\frac{\rho_p
d_p^2}{18\mu}
\end{equation}

If we suppose that the flow velocity is constant and the initial droplet 
velocity is zero the  solution of the previous equation is:


\begin{equation}
v=u(1-e^{-t/\tau_p})
\end{equation}

We can observe that the droplet velocity
approaches quickly to the fluid velocity for decreasing the response time.
This proprierties depends on the fluid time scale and 
 is well described by the Stokes number that takes into
account the information about the flow field too.
Specifically, the Stokes number is a measure of the droplet response to the surroundig
velocity field.
%The Stokes number is defined by the ratio between the particle response time and
%the time characteristic of the flow field.
For instance, we can immagine a droplet in a vortex with a
scale $L_f$ and velocity $U_f$ (order of
magnitude)  with a characteristic time $\tau_f=L_f/U_f$.

The Stokes number related to this scale is by definition:

\begin{equation}
St_{p_f}=\frac{\tau_p}{\tau_f}
\end{equation}

Thus, we can write the equation (Eq. \ref{eq:partlib3}) in dimensionless form using
length scale $L_f$ and velocity scale $U_f$:

\begin{equation}\label{eq:partlib4}
\frac{d\tilde{v}}{d\tilde{t}}=\frac{1}{St_{p_f}}(\tilde{u}-\tilde{v})
\end{equation}

where $\tilde{u}$, $\tilde{v}$, $\tilde{t}$ are the dimensionless quantities respectively of $u$,
$v$, $t$.
The solution of the previous equation, plotted in Fig. \ref{fig:resp}, is:

\begin{equation}
\tilde{v}=\tilde{u}(1-e^{-\tilde{t}/St_{p_f}})
\end{equation}



\begin{figure}[!h]
\begin{center}
\includegraphics[width=.6\textwidth,angle=0]{./figs/response.jpg}
\caption{\small Comparison between flow and droplet velocities for three Stokes
number: $St_{p_f}=10^{-1}$, $St_{p_f}=5\cdot 10^{-2}$, $St_{p_f}=10^{-2}$}
\label{fig:resp}

\end{center}
\end{figure}

The droplet is selectively sensitive to the flow velocity 
induced by the turbulence. Specifically, the droplet with very small
Stokes number will simply be a flow tracers $St_{p_f}<<1$. For increasing the Stokes number,
the droplet trajectory will diverge from the flow stream-line until the droplet 
motion will be completely independent from the surrounding flow $St_{p_f} >> 1$
(Fig. \ref{fig:interaction}). In several
previous works it is shown that the droplets are preferentially dispersed if the
Stokes number has order one \cite{Sq90}.
Thus, at unity Stokes number corrsponds the vortical structures responsible 
for the topological configuration of the droplets system.

\begin{figure}[!h]
\begin{center}
\includegraphics[width=1.0\textwidth]{./figs/interaction.png}
\caption{\small Qualitatively description of the interaction between
particle and vortices.}
\label{fig:interaction}
\end{center}
\end{figure}




The Stokes number can
be estimated once the velocity scale and the length scale  responsible
for the maximum interaction between vortical structures and droplets has been
modelled.
We analyse the case of  isotropic and homogeneous turbulence that
 is the turbulence dynamic far from the boundaries.

The turbulence dynamics in the case of isotropic and homogeneous turbulence is
described by Kolmogorov theory. This theory is based on the following
hypothesis: i) For high Reynolds numbers (ratio between the inertial and the
viscous forces) the small turbulent structures, developed in a turbulent flow,
are statistically isotropic; ii) For high Reynolds numbers the main properties
of the small scales are the same for every kind of turbulent flows. The
behavior of the small
scales is described by the viscosity $\nu$ and by the dissipation energy
$\epsilon$ iii) The dynamics of the structures with dimension  between the
large scale and the dissipative one (inertial range) are dominated only by
$\epsilon$.

 We can write using dimensionless analysis and the hypothesis ii) the
expressions for the dissipative scales $\eta$, $U_k$, $\tau_k$ respectively
for length, velocity and time:

\begin{equation}\label{viscous0}
 \eta=\left(\frac{\nu^3}{\epsilon}\right)^{1/4},\hspace{0.5cm}U_{k}=(\nu\epsilon)^{1/4}\hspace{0.5cm}\tau_{k}=\left(\frac{\nu}{\epsilon}\right)^{1/2};
  \end{equation}

In the case of stationary flow  $\epsilon$ is the same of the amount of energy
at the large scales; then, $\epsilon=U_f^3/L_f$ where $U_f$ and $L_f$ are respectively the
velocity and the length at large scales. The previous expression of $\epsilon$
does not take into account the viscosity because at the large scale the cascade
of energy is dominated by the inertial terms responsible only for the transport
of energy. At the large scale the dissipative effects due to the viscous terms
are negligible.
The relations between the velocity
$U_{f}$, the length $L_f$ and the time $\tau_{f}$ at the large scales
 are related to the Kolmogorov scales, $\eta$, $U_k$, $\tau_k$, as follows:
 \begin{equation}\label{viscous1}
 \frac{\eta}{L_f}=Re_f^{-3/4},\hspace{0.5cm}\frac{U_{k}}{U_f}=Re_f^{-1/4}\hspace{0.5cm}\frac{\tau_{k}}{\tau_f}=Re_f^{-1/2};
 \end{equation}
 where $Re_f=(U_fL_f)/\nu$ is the Reynolds number evaluated at larger vortical scales.
 We use equations (\ref{viscous1}) to estimate
  the Stokes number  based on the Kolmogorov scales
  $St_{p_k}$  as function of the Stokes number based on the large
  eddy time scale.

  \begin{equation}\label{Stk}
  St_{p_k}=\frac{\tau_p}{\tau_k}=\frac{\tau_p}{\tau_f}\frac{\tau_f}{\tau_k}=St_{p_f}Re_f^{1/2}
  \end{equation}


 The analogue relations  between the times $\tau_{f}$ (large scale) and $\tau_r$
 (inertial range) and the velocities $U_f$ (large scale) and $U_r$ (inertial
 range) based on the hypothesis iii) are:


\begin{equation}
\frac{U_r^3}{r}=\epsilon =\frac{U_f^3}{L_f}\Longrightarrow
\frac{U_f}{U_r}=\left(\frac{L_f}{r}\right)^{1/3}
\end{equation}


  \begin{equation}\label{inertial1}
  \tau_r=\frac{r}{U_r}\Longrightarrow\frac{\tau_f}{\tau_r}=\left(\frac{L_f}{r}\right)^{2/3}
  \end{equation}
  where $r$ is the  characteristic scale of the inertial  range.



The Stokes number  based on the generic dimensionless eddy size $r=r/L_f$
is:

  \begin{equation}\label{Str1}
     St_{p_r}=\frac{\tau_p}{\tau_r}=\frac{\tau_p}{\tau_k}\frac{\tau_k}{\tau_f}\frac{\tau_f}{\tau_r}=St_{p_k}Re_f^{-1/2}
     r^{-2/3};\hspace{0.3cm}
            \end{equation}

\subsection{The droplets collision}


To complete the analysis about the control parameter of dispersion of the droplet 
in fluids we describe the dilute and dens flows.
A dilute flow is one in which the droplet motion is controlled by the fluid
forces (drag and lift). A dense flow is one in which the droplet motion is
controlled by collision. A quantitative estimate of the dilute or dense nature
of the flow can be made by comparing the ratio of momentum response time of a
droplet to the time between collisions.

Thus the flow can be consider dilute if:

\begin{equation}
\frac{\tau_f}{\tau_c}<1
\end{equation}

where $\tau_c$ is the average time between droplet-droplet collisions because
the droplets have sufficient time to respond to the local fluid dynamic forces
before the next collision. On the other hand, if

\begin{equation}
\frac{\tau_f}{\tau_c}>1
\end{equation}


then the droplet has no time to respond to the fluid dynamic forces before the
next collision and the flow is dense.
The time between collisions can be estimated from the classic equations for
collision frequency.




\begin{figure}[!h]
\begin{center}
\includegraphics[width=.6\textwidth,angle=0]{./figs/PartColl.jpg}
\caption{\small Schematic of the droplet-droplet collision}
\label{fig:PartColl}
\end{center}
\end{figure}

Consider a group of droplets with uniform diameter $d_p$ as shown in figure
Fig. \ref{fig:PartColl} through which one droplet is traveling with a relative velocity $v_r$
with respect to the other droplets. In a time $\delta t$, the one droplet will
intercept all the droplet in tube with radius $2d_p$ and length $v_r\delta t$.
The number of droplets in this tube is:

\begin{equation}
\delta n=n\pi d_p^2 v_r\delta t
\end{equation}

where n is the number density of droplets. Thus the collision frequency is:

\begin{equation}
f_c=n \pi d_p^2 v_r
\end{equation}

and the time between collisions is:

\begin{equation}
\tau_c=\frac{1}{f_c}=\frac{1}{n\pi d_p^2v_r}
\end{equation}

Thus the time ratio $\tau_f/\tau_c$ can be expressed as:

\begin{equation}
\frac{\tau_f}{\tau_c}=\frac{n\pi\rho_pd_p^4v_r}{18\mu_f}
\end{equation}

However, the product of the number density and the mass of an individual
droplet is equal to the bulk density of the dispersed phase so the above
equation can be written as:

\begin{equation}
\frac{\tau_f}{\tau_c}=\frac{\overline{\rho_p}d_pv_r}{3\mu_f}
\end{equation}

Thus the flow would be considered dilute if:

\begin{equation}
\frac{\overline{\rho_p}d_pv_r}{3v_r}<1
\end{equation}


%We use, for the droplet equations, a model with only inertia, weight and
%steady drag forces, because the other forces can be neglected \cite{Maxey, Camp}.
%Particle momentum equation, based on the previous hypothesis, is written as follows:

%\begin{equation}
%m_p\frac{d\textbf{v}}{dt}=f3\pi\mu
%d(\textbf{u}-\textbf{v})+m_p\textbf{g};\hspace{1cm}\frac{d\textbf{x}}{dt}=\textbf{v}
%\end{equation}


%\begin{equation}
%f=1+0.15Re_d^{0.687}
%\end{equation}
%\begin{equation}
%\hspace{0.5cm}Re_p=\frac{|\textbf{u}-\textbf{v}|d_p}{\nu}
%\end{equation}
%We use the drag correction $f$  obtained by Shiller and
%Naumann \cite{Shi33}.

%***MORE

%Time solution  is obtained integrating the droplet velocity equation and the droplet position equation.
%The flow velocities on the droplets positions are calculated by interpolating velocities from the closest 8 grid points.
%This interpolation scheme has the same 2nd order accuracy in space of the flow field solution.
%The implicit scheme avoid the instability problem due to explicit scheme that is usually solved using an slightly time steps below the critical value
%increasing the time consuming to solve the droplet velocity equation.


==> Methods.tex <==
\section{Implicit and explicit interface representation}

In three space dimension a closed surface separate the whole domain $\Omega$ into the inside domain $\Omega^-$ 
and the outside domain $\Omega^+$. The border between the inside domain and the outside domain is called the interface $\partial\Omega$.
In an explicit interface representation one explicitly writes the points that belong to the interface  when defining $\partial\Omega$.
In three spatial dimensions the explicit representation can be quite difficult to discretize. One needs to choose a number 
of points on the two-dimensional surface and record their connectivity. In two spatial dimensions, connectivity was determined based on the 
ordering, i.e. $\textbf{x}_i$ is connected to $\textbf{x}_{i-1}$ and $\textbf{x}_{i+1}$. In three spatial dimensions connectivity is 
less straightforward. If the exact surface and its connectivity are known, it is simple to tile the surface with triangles whose vertices 
lie on the interface and whose edges indicate connectivity. 
On the other hand, if connectivity is not known, it can be quite difficult to determine, and even some of the 
most popular algorithms can produce inaccurate surface representation,e.g, surfaces with holes.
Moreover, in three spatial dimensions the interface merging and pinching are complex, leading to a number of difficulties 
including hole in the surface.
One of the nicest properties of implicit surfaces is that connectivity does not need to be determined for the discretization.
The most powerful aspect of implicit surfaces is that it is straightforward to go from two spatial dimensions to three spatial dimensions.
An implicit interface representation defines the interface as the isocontour of some function.
For instance, the zero isocontour of  

\begin{equation}
\phi (\textbf{x})=x^2+y^2+z^2-R_s^2
\end{equation}



\begin{figure}[!h]
\begin{center}
\includegraphics[width=.3\textwidth,angle=0]{./figs/snapshot.png}
\caption{\small Implicit representation of a sphere with interface defined by
$\phi=0$.}
\label{fig:snapshot.png}
\end{center}
\end{figure}





is the set of all points where $\phi (\textbf{x})=0$ on ($\partial\Omega$).  
Implicit interface representation include some very powerful geometric tools. 
For instance, since we have designated the $\phi (\textbf{x})=0$ isocontour 
as the interface, we can determine which side of the interface a point is on simply by looking at the local sign of $\phi$. The inner region
and the outer region is defined by $\phi (\textbf{x})<0$ and $\phi (\textbf{x})>0$, respectively.
With an explicit representation of the interface it can be difficult to determine whether a point is inside or outside the interface.
A standard procedure for doing this is to cast a ray from the point to some far-off place that is known to be outside the interface.
Then if the ray intersect the interface an even number of times, the pint is outside the interface. Otherwise, the ray intersect the interface an odd 
number of times, and the point is inside the interface.
Implicit functions make both simple Boolean operations and more advanced constructive solid geometry operations easy to apply.
If $\phi_1$ and $\phi_2$ are two different implicit functions, then $\phi (\textbf{x})=min(\phi_1 (\textbf{x}),\phi_2 (\textbf{x}))$ 
is the implicit function representing the union of the inner regions of $\phi_1$ and $\phi_2$. 
Similarly, $\phi (\textbf{x})=max(\phi_1 (\textbf{x}),\phi_2 (\textbf{x}))$ is the implicit function representing the 
intersection of the inner regions of $\phi_1$ and $\phi_2$. 
The complement of $\phi_1(\textbf{x})$ can be defined by $\phi (\textbf{x})=-\phi_1(\textbf{x})$. 
Also, $\phi (\textbf{x})=max(\phi_1 (\textbf{x}),-\phi_2 (\textbf{x}))$ represents the region obtained by subtracting the interior of $\phi_2$ 
from the interior of $\phi_1$.

\subsection{Normal to the interface and mean curvature}

The gradient of the implicit function is defined as:

\begin{equation}
\nabla\phi =\left(\frac{\partial\phi}{\partial x}, \frac{\partial\phi}{\partial y}, \frac{\partial\phi}{\partial z}\right)
\end{equation}


The gradient $\nabla\phi$ is perpendicular to the isocontours of $\phi$ 
 Therefore, $\nabla\phi$ evaluated at the interface is a vector that points in the same direction as the local unit (outward) normal $\textbf{n}$ 
 to the interface. Thus, the unit (outward) normal is:

\begin{equation}\label{eq.norm}
\textbf{n}=\frac{\nabla\phi}{|\nabla\phi|}
\end{equation}

for points on the interface.


The mean curvature of the interface is defined as the divergence of the normal $\textbf{n}=(n_1, n_2, n_3)$,

\begin{equation}
k=\nabla \cdot \textbf{n}=\frac{\partial n_1}{\partial x}+\frac{\partial n_2}{\partial y}+\frac{\partial n_3}{\partial z}
\end{equation}

so that $k>0$ for convex regions, $k<0$ for concave regions, and $k=0$ for a plane.

Using the definition of normal vector we obtain:

\begin{equation}\label{eq.curv}
k=\nabla\cdot\left(\frac{\nabla\phi}{|\nabla\phi|}\right)
\end{equation}




\subsection{Signed distance function}
Smoothness of the $\phi$ is a desiderable property especially in  using numerical approximations.
Signed distance functions are a subset of the implicit functions $\phi$. 
We define signed distance functions to be positive on the outer, negative on the inner, and zero on the boundary. 
An extra condition of $\nabla\phi (\textbf{x})=1$ is imposed on a signed distance function.
The signed distance function turns out to be a good choice, since steep and flat gradients as well as rapidly changing features are avoided as much
as possible.
A distance function $d(\textbf{x})$ is defined as:

\begin{equation}
d(\textbf{x})=min(|\textbf{x}-\textbf{x}_i|)\hspace{0.5cm}\mbox{for all }\textbf{x}_i\in\partial\Omega
\end{equation}

implying that $d(\textbf{x})=0$ on the boundary where $\textbf{x}\in\partial\Omega$. 
Geometrically, $d$ may be constructed as follow. If $\textbf{x}\in\partial\Omega$, then $d(\textbf{x}=0)$. Otherwise, for 
a given point $\textbf{x}$, find the point on the boundary set $\partial\Omega$ closest to $\textbf{x}$, and label this point $\textbf{x}_c$.
Then $d(\textbf{x})=|\textbf{x}-\textbf{x}_c|$.
Evaluating $-\nabla d$ at any point on the line segment from $\textbf{x}$ to $\textbf{x}_c$ gives a vector that points from $\textbf{x}$ 
to $\textbf{x}_c$. Furthermore, since d is an Euclidean distance,

\begin{equation}\label{eq.d}
|\nabla d|=1
\end{equation}

which is intuitive in the sense that moving twice as close to the interface gives a value of $d$ that is half as big.
The above argument leading to equation (Eq. \ref{eq.d}) is true for any $\textbf{x}$ as long as there is a unique closest point $\textbf{x}_c$.

A signed distance function is an implicit function $\phi$ with $|\phi (\textbf{x})|=d(\textbf{x})$ for all $\textbf{x}$. 
Thus $\phi(\textbf{x})=d(\textbf{x})=0$ for all $\textbf{x}\in\partial\Omega$, $\phi (\textbf{x})=-d(\textbf{x})$ for all $\textbf{x}\in\Omega^-$, 
and $\phi(\textbf{x})=d(\textbf{x})$ for all $\textbf{x}\in\Omega^+$. Signed distance functions share all the properties of implicit functions discussed
in the last chapter. 
Signed distance functions are the best candidates for implicit representation of interfaces. 
 There are a number of new properties that only signed distance function posses.
This the normalization 
 in equations (Eq. \ref{eq.norm}) and (Eq. \ref{eq.curv}) is removed since $|\nabla\phi |=1$ everywhere. 
Equation  (Eq. \ref{eq.norm}) simplifies to 

\begin{equation}
\textbf{n}=\nabla\phi
\end{equation}

for the local unit normal. Equation (Eq. \ref{eq.curv})  simplifies for the three spatial dimensions case to

\begin{equation}
k=\frac{1}{2}\nabla^2\phi
\end{equation}


\subsection{Front Tracking}


Level-Set and Front Tracking methods add dynamics to implicit surfaces. 
Suppose that the velocity of each point on the implicit surface is given as $\textbf{v}(\textbf{x})$ and assume that $\textbf{v}(\textbf{x})$ 
is known for every point $\textbf{x}$ with $\phi (\textbf{x})=0$.
Given this velocity field we wish to move all the points on the surface with this velocity.
The simplest way to do this is to solve the ordinary differential equation:

\begin{equation}
\frac{d\textbf{x}}{dt}=\textbf{v}(\textbf{x})
\end{equation}

for every point on the discretize front.
This is the Lagrangian formulation of the interface evolution equation. 
Unfortunately, even the most trivial velocity fields can cause large distortion of boundary elements (triangles), and the accuracy 
of the method can deteriorate quickly if one does not periodically modify the discretization in order to account for these deformation 
by smoothing and regularizing inaccurate surface elements. 
In addition to dealing with element deformations, one must decide how to modify the interface discretization when topology changes.
These methods of detaching and re-attaching boundary elements can quickly become rather complicated.
The use of the Lagrangian of the interface motion with numerical techniques for smoothing, regularization are collectively referred 
to as front tracking methods.

\subsection{Advection of the interface using Level-Set method}

In order to avoid problems with instabilities, deformation of surfaces elements, and complicated procedures for topological repair of interfaces, 
we use our implicit function $\phi$ both to represent the interface and evolve the interface. 
In order to define the evolution of our implicit function $\phi$ we use the simple advection equation:

\begin{equation}
\phi_t+\textbf{v}\cdot\nabla\phi =0
\end{equation}

where the $t$ subscript denotes a temporal partial derivative in the time variable $t$.
This partial differential equation defines the motion of the interface where $\phi\textbf{x}=0$.
 It is and Eulerian formulation of the interface evolution, since the interface is captured by the implicit function $\phi$ 
 as proposed to being tracked by interface elements as was done in the Lagrangian formulation.
 The previous equation is sometimes referred to as level set equation; it was introduced for numerical interface evolution 
 by Osher and Sethian \cite{OsSe}.

\section{Set-up of the liquid jet simulation}

The Level-Set method is used to identify the spatial evolution of the liquid jet. 
The injection of the spray is modelled enforcing a prescribed curvature of the liquid phase according to 
the diameter of the injector and to the initial angle of the spray.
Assuming the injector diameter $d_i$ and the initial angle of the spray $\alpha_i$ the blow injection is located at a 
distance from the orifice of the injector equal to:

\begin{equation}
h_i=\frac{d_i}{2}tg\left(\frac{\alpha}{2}\right)
\end{equation}

The radius of the sphere is defined by $R_s=1/k^0_{spray}$ where $k^0_{spray}$ is the initial curvature of the spray detaching from the injector.
The center of the sphere is define by $(x_s,y_s,z_s)$ where $y_s=y_i$ and $x_s=x_i$, while $z_s$ depend on $k^0_{spray}$ 
and $\alpha_i$.
Thus, $z_s$ is equal to:

\begin{equation}
z_s=z_i-\sqrt{R_s^2-\frac{d_i^2}{4}}+h_i
\end{equation}

\begin{equation}
z_s=z_i-\sqrt{R_s^2-\frac{d_i^2}{4}}+\frac{d_i}{2}tg\left(\frac{\alpha_i}{2}\right)
\end{equation}


\begin{figure}[!h]
\begin{center}
\includegraphics[width=.6\textwidth,angle=0]{./figs/spray.png}
\caption{\small Initial level-set isocontour.}
\label{fig:spray.png}
\end{center}
\end{figure}



The liquid jet has been treated with a Lagrangian poit of view. It is
rapresented by small droplets coupled with the surrounding fluid (air) mechanically.
This represatation takes into account the instability effects at the liquid jet
interface since each particle is sensitive to the fluctuations of the
velocity field.
In order to reproduce the lagrangian description of the liquid jet the motion of 
each particle has to be like a flow tracer. The droplet diameter has been 
chosen enforcing the Stokes number related to the dissipative scale equal to one.
 

\begin{equation}
St_{pk}=\frac{\tau_p}{\tau_f}Re_f^{-1/2}=1
\end{equation}

\begin{equation}
d_{p_{max}}=\frac{18\mu}{\rho_p}\frac{d_i}{U_f}Re_f^{-1/2}
\end{equation}

where $d_i=1.58\cdot10^{-4}$ $[m]$ is the diameter of the injector, $U_f=27$ $[m/s]$ the velocity and $Re_f=4.3 10^3$ 
the Reynolds number of the liquid phae into the injector, the droplet density is $\rho_p=10^3$ $[Kg/m^3]$.
According to this set-up the droplet diameter is equal to $d_{p_{max}}=6.9\cdot 10^{-9}$ $[m]$, thus the liquid jet has been 
discretized using droplet wuth diameter $d_p=10^{-9}$ $[m]$.

The interface is organized in an elongated structure with hinomogenous shape.


\begin{figure}[!h]
\begin{center}
\includegraphics[width=.2\textwidth,angle=0]{./figs/jet.png}
\caption{\small Interface of the liquid jet.}
\label{fig:fractal.png}
\end{center}
\end{figure}

The interface topology is descibed with the fractal dimension. 
This feature will be deeply described in the
next section. The fractal dimension is the control parameter 
of the model of the primary break-up since it is the integarl measure of 
the distorsion of the liquid jet. 


\section{Fractal dimension of the liquid jet interface}



The dimension of a line, a square, and a cube are one, two, and
three respectively. And, we can measure the distance, area, and volume of those
objects as well. 
If we take an object residing in Euclidean dimension $D$ and reduce its linear
size by $1/r$ in each spatial direction, its measure (length, area, or volume)
would increase to $N=r^D$ times the original. This is pictured in the next figure. 


\begin{figure}[!h]
\begin{center}
\includegraphics[width=1.0\textwidth,angle=0]{./figs/fractal.png}
\caption{\small Exaples of figures with integer dimension.}
\label{fig:jet.png}
\end{center}
\end{figure}

We consider $N=r^D$, take the log of both sides, and get 
\begin{equation}
log(N) = D log(r)
\end{equation}
If we solve for D. 
\begin{equation}
D = log(N)/log(r) 
\end{equation}

The point: examined this way, D need not be an
integer, as it is in Euclidean geometry. Fractals, which are irregular geometric
objects, have a fractional dimension. This generalized treatment of dimension is named after the
German mathematician, Felix Hausdorff. 


Fractal Dimension allows us to measure the degree of complexity by evaluating
how fast our measurements increase or decrease as our scale becomes larger or
smaller.

Before explaining dimension measuring algorithms (box counting), we must explain how a power
law works. Essentially, data behave with a power law relationship if they fit
the following equation: $N=c\cdot r^D$ where $c$ is a constant. One way to determine if
data fit a power law relationship is to plot the log(N) versus the log(r). If
the plot is a straight line, then it is a power law relationship with slope D.

To calculate the box-counting dimension, we need
to place the geometry on a grid. The x-axis of
the grid is s where s=1/(width of the grid). 
For example, if the grid is 240 blocks tall by 120
blocks wide, s=1/120. Then, count the number of
blocks that the picture touches. Label this
number N(s). Now, resize the grid and repeat the
process. Plot the values found on a graph where
the x-axis is the log(s) and the y-axis is the
log(N(s)). Draw in the line of best fit and find
the slope. The box-counting dimension measure is
equal to the slope of that line.

The Box-counting dimension is widely
used since
the box-counting dimension can measure geometry
that are not self-similar (and most real-life
applications are not self-similar).


The fractal dimension of the liquid jet has been computed using the numerical simulation
in the two dimensions case. The extension to the three dimension case will be future development.
The fractal dimension has been computed using the box counting method via the best fit of the 
data provided processing the axial section of the liquid jet.




\begin{figure}[!h]
\begin{center}
\includegraphics[width=.5\textwidth,angle=0]{./figs/box_count_log_2d.jpg}
\caption{\small Best fit of the fractal dimension using the box counting method.}
\label{fig:box_count_log_2d.jpg}
\end{center}
\end{figure}

The slope of the best fit is equal to 1.22 and it represent the degree of complexity of the 
liquid jet surface.

The fractal dimension provided by the numerical simulation plays a fundamental role in the primary breakup model
since it is related to the forcing of the interface induced by the turbulence generated during the injection.




Specifically, the initial diameter of the drops for the Blob model depends on the fractal dimension of the interface according to the following relation:


\begin{equation}
d_p=\frac{6\sigma}{C\left(\Delta p-\frac{8}{\pi^2}\frac{m^2}{\rho d_h^4C_d^2\Delta t^2}\right)+\frac{4\sigma D}{d_hC_d}}
\end{equation}



\begin{table}[!h]
\begin{tabular}{lll}
\hline
C  &    dissipation coefficient & [adim]\\
M  &    injected mass & [kg]\\
Cd  &   outflow coefficient & [adim]\\
$d_h$    &  hole diameter& [m]\\
D     &  fractal parameter &[adim]\\
$d_p$    &  droplets diameter &[m]\\
p   & pressure drop between the injector and the injection environment& [Pa]\\
$\rho$   &    liquid density &[kg/m3]\\
$\sigma$  &    superficial tension &[N/m] \\
\hline
\end{tabular}
\caption{Parameter of the model for the droplet diameter}
\end{table}


This model has been tested against experimental results as it is showed in the following picture:



\begin{figure}[!h]
\begin{center}
\includegraphics[width=1.\textwidth,angle=0]{./figs/poster2.jpg}
\caption{\small }
\label{fig:poster2.jpg}
\end{center}
\caption{\small Probability function of deroplet size.}
\end{figure}

All the steps to predict the droplet diameter $d_p$ have been sketced:


\begin{figure}[!h]
\begin{center}
\includegraphics[width=1.2\textwidth,angle=0]{./figs/poster4.png}
\caption{\small }
\label{fig:poster4.png}
\end{center}
%\caption{\small Probability function of deroplet size.}
\end{figure}
















==> Numerical.tex <==
\section{Numerical solution of the equations governing the flow}

%\begin{figure}[ht]
%\includemovie[
%poster, text={\small(Loading 3D.avi)}
%]{6cm}{6cm}{3D.avi}
%\end{figure}
Kiva is a numerical code for the computation of three-dimensional, chemically reactive fluid flow with sprays. 
A sthocastic particle method is used to calculate evaporating liquid sprays, including the effects of droplet collisions and aerodynamic breakups.
Kiva solves the unsteady equations of motion of a turbulent flow coupled to the equation for a spray. The gas-phase solution procedure 
is based on a finite volume method.
The finite volume method uses the integral form of the conservative equations applyed to the control volume $V_0$ with a boundary surface $S_0$ and 
the unity normal vector pointing outword to the surface $S_0$ defined by $\textbf{n}$: 

\begin{equation}
\int_{V_0}\frac{\partial\rho}{\partial t}dV+\int_{S_0}\rho\textbf{u}\cdot\textbf{n}dS=0
\end{equation}	


\begin{equation}
\int_{V_0}\frac{\partial\rho\textbf{u}}{\partial t}dV+\int_{S_0}\rho\textbf{u}\textbf{u}\cdot\textbf{n}dS
=-\int_{S_0}p\textbf{n}dS+\int_{S_0}\mu\nabla^2\textbf{u}\cdot\textbf{n}dS+\int_{V_0}\rho\textbf{g}dV+\int_{V_0}\textbf{f}_{spray}dV
\end{equation}

where $\rho$,  $\mu$ are the density and the dynamic viscosity respectively. The flow velocity is $\textbf{u}$, the gravity vector is $\textbf{g}$ 
, the flow pressure is $p$, the time is $t$ and the feedback forcing induced by the spray is $\textbf{f}_{spray}$

The solution domain is subdivided into a finite number of contiguous 
control volumes, and the conservation equations are applied to each control volume.
At the centroid of each control volume lies a computational node at which the variables values are to be calculated.
Interpolation is used to express variable values at the control volume surface in terms of the nodal values. 
Surface and volume integrals are approximated using suitable quadrature formulae. 
As a result, one obtains an algebraic equation for each control volume, in which number of neighbor nodal values appear.

The finite volume method can accomodate any type of grid, so it is suitable for complex geometries. 
The grid defines only the control volume boundaries and need not be related to a coordinate system. 
The method is conservative by construction, so long as surface integrals (which represent convective and diffusive fluxes) 
are the same for the control volumes sharing the boundary.
The finite volume approach is pherhaps the simplest to understand and to program. All terms that need be approximated have physical meaning 
which is why it is popular with engineers. The disavantage of the finite volume methods is that methods of order higher than second are 
difficult to develop in three space dimensions. 
The Cartesian components of velocity vector are stored at cell verticies and the transient solution is marched out in a sequence 
of finite timesteps.

The effect of turbulence is take into account with a standard version of $k-\epsilon$ turbulence model modified to include spray-turbulence interaction.
Evaporating liquid sprays are represented by a discrete-particle technique, in which each computational particle represent a number of droplets 
of identical size, velocity and temperature.
The particles and fluid interact by exchanging mass, momentum, and energy. 
The momentum exchange is treated by implicit coupling procedures to avoid the prohibitively
small timesteps that would otherwise be necessary. Accurate calculation of mass and
energy exchange is ensured by automatic reductions in the timestep when the exchange
rates become large. Turbulence effects on the droplets are accounted.
When the timestep is smaller than the droplet turbulence correlation time, a fluctuating
component is added to the local mean gas velocity when calculating each particle’s mass,
momentum, and energy exchange with the gas. When the timestep exceeds the turbulence
correlation time, turbulent changes in droplet position and velocity are chosen randomly
from analytically derived probability distributions for these changes. Droplet
collisions and coalescence are accounted. Volume displacement and thick spray effects on the
exchange rates are neglected.


%\subsection{Temporal differencing}

The temporal differencing is performed with respect to a sequence of discrete times
$t^n$(n = O, 1,2, ...). The time interval $\Delta t^n = t^{n+1}-t^n$ is the time-step, and the integer n is
the cycle number. The latter is displayed as a superscript, so that $Q^n$ denotes the difference
approximation to the quantity $Q$ at time $t^n$. When $\Delta t$ appears without a superscript,
$\Delta t^n$ is understood. The difference approximation to the derivative $\partial Q/\partial t$ is the first-order
expression $(Q^{n+1}-Q^n)/\Delta t$.
A cycle is performed in two steps. 
Phase A is a calculation of spray droplet collision and oscillator breakup terms and
mass source terms due to the spray. Phase B calculates in a
coupled, implicit fashion the pressure gradient in the
momentum equation and velocity dilatation terms in mass equations, the
spray momentum source term, and the terms due to diffusion of mass and momentum. 
Phase B also calculates the remaining source terms in the turbulence equations.

%\subsection{Spatial differencing}

Spatial difference approximations are
constructed by the control-volume or integral-balance approach, which largely preserves
the local conservation properties of the differential equations.
The spatial region of interest is subdivided into a number of small cells or zones,
the corners of which are the vertices. Together, the cells constitute the mesh with
respect to which spatial differences are formed. In the general case, the cells are asymmetrical. 
The cells are indexed by integers $(i,j,k)$, which may be regarded as coordinates in logical
space.
%Since each face is common to two cells, there are three independent faces per cell.
%These are conventionally taken to be the left, front, and bottom faces of the cell as viewed
%from the perspective of **** Fig. 2. 
%These faces are shown in ****Fig. 4. 
The conventional direction
of the vector area elements of the cell faces is outward from the cell.
%*****INSERT FIGURE********
%where subscripts f, L and b refer respectively to the left,front, and bottom faces. When needed,
%the subscripts r, d, and t will be used to refer respectively to the right, back and
%top faces of a computational cell. 
%These area projections enable us to define area vectors
$\textbf{A}_i$ associated with the faces $i$ of each regular cell. It is convenient to associate $\textbf{A}_i$ with
both the face and the cell; so that $\textbf{A}_i$ may be considered to always point outward from the
cell under consideration. Thus, for a given face, the sign of $\textbf{A}_i$ depends on the side of the
face from which it is viewed.

In the finite-difference approximations of KIVA, velocities are located at the vertices, so that

\begin{equation}
\textbf{u}_{(i,j,k)}=\textbf{u}(x_{(i,j,k)}, y_{(i,j,k)}, z_{(i,j,k)})
\end{equation}

Scalar quantities are located at cell centers:

\begin{equation}
Q_{i,j,k}=Q(x^c_{(i,j,k)}, y^c_{(i,j,k)}, z^c_{(i,j,k)})
\end{equation}


where $Q$ is a general scalar quantities. Quantities needed at points where they are
not located are obtained by averaging neighboring values.
Spatial differences are usually performed by integrating the differential term 
over the volume of a cell. Volume integrals of gradient
or divergence terms are  converted into surface area integrals using the divergence
theorem. The volume integral of a time derivative maybe related to the derivative
of the integral by means of Reynolds’ transport theorem.  Volume and surface area integrals
are  performed under the assumption that the integrands are uniform within
cells or on cell faces. Thus area integrals over surfaces of cells become sums over cell faces:

\begin{equation}
\int_\textbf{S}\textbf{F}d\textbf{A}=\sum_k\textbf{F}d\textbf{A}
\end{equation}




==> biblio.tex <==
\begin{thebibliography}{99}


%\bibitem{ShNa} Shiller, L., Naumann, A., 1933. \"Uber die grundlegenden Berechungen bei der Schwerkraftaufbereitung. Ver. Deut. Ing. 77, 318.

\bibitem{Front1} Unverdi, S.O., Tryggvason, G., 1992. A front-tracking method for viscous, incompressible multi-ﬂuid ﬂows. J. Comput. Phys. 100, 25–37.

\bibitem{Vol1} Gueyﬃer, D., Li, J., Nadim, A., Scardovelli, S., Zaleski, S., 1999. Volume of Fluid interface tracking with smoothed surface stress methods
 for three-dimensional ﬂows. J. Comput. Phys. 152, 423–456.

\bibitem{Level1} Osher, S., Sethian, J.A., 1988. Fronts propagating with curvature-dependent speed: algorithms based on Hamilton–Jacobi formulations.
       J. Comput. Phys. 79, 12–49.

\bibitem{Level2} Osher, S., Fedkiw, R., 2003. Level set methods and dynamic implicit surfaces. In: Applied Mathematical Sciences, vol. 153. Springer, New
          York.

\bibitem{OsSe} Osher, S., Sethian, J., 1988. Fronts propagation with curvature dependent speed: algorithms based on
Hamilton-Jacobi formulations. J. Comput. Phys. 79, 12–49.

\bibitem{Sq90} Squires, K. D., Eaton, J. K., 1990. Particle response and turbulence modification in isotropic turbulence. Phys. Fluids A, 
(2)1192-1203.

\bibitem{Elg93} Elghobaschi, S., Truesdell, G. C., 1993. On the two-way interaction between homogeneous turbulence and dispersed solid particles. 
Phys. Fluids A, (5)1790-1810.

\bibitem{Boi98} Boivin, M., Simonin, O., Squires, K., 1998. Direct numerical simulation of turbulence modulation by particles in 
isotropic turbulence. J. Fluid Mech., (375)235-263.

\bibitem{Maxey} Maxey, M. R., Riley, J. J., 1983. Equation of motion for a small rigid sphere in a nonuniform flow. Phys. Fluids, 26(4)883-889.

\bibitem{Camp} Campolo, M., Salvetti, M. V., Soldati, A., 2004. Mechanisms for microparticle dispersion in a jet in crossflow. 
AIChE Journal, 51(1)28-43.

\bibitem{Shi33} Shiller, L., Naumann, A., 1933. \"Uber die grundlegenden berechungen bei der schwerkreftaufbereitung. Ver Deut. Ing., (77)318.

\bibitem{Elg} Elghobaschi, S., Truesdell, G. C., 1992. Direct simulation of particle dispersion in a decaying isotropic turbulence. J. Fluid Mech., 
(242)655-700.


\end{thebibliography}


